EVHA: Explainable Vision System for Hardware Testing and Assurance -- An Overview

Due to the ever-growing demands for electronic chips in different sectors the semiconductor companies have been mandated to offshore their manufacturing processes. This unwanted matter has made security and trustworthiness of their fabricated chips concerning and caused creation of hardware attacks. In this condition, different entities in the semiconductor supply chain can act maliciously and execute an attack on the design computing layers, from devices to systems. Our attack is a hardware Trojan that is inserted during mask generation/fabrication in an untrusted foundry. The Trojan leaves a footprint in the fabricated through addition, deletion, or change of design cells. In order to tackle this problem, we propose Explainable Vision System for Hardware Testing and Assurance (EVHA) in this work that can detect the smallest possible change to a design in a low-cost, accurate, and fast manner. The inputs to this system are Scanning Electron Microscopy (SEM) images acquired from the Integrated Circuits (ICs) under examination. The system output is determination of IC status in terms of having any defect and/or hardware Trojan through addition, deletion, or change in the design cells at the cell-level. This article provides an overview on the design, development, implementation, and analysis of our defense system.

==> 02_Related_Works.tex <==
\section{Related Works}\label{sec:related_works}
In this section, the related published works in the area of hardware security based on the proposed attacks and defenses are discussed.
    
\subsection{Hardware Security - Attacks}
As IC production operations are increasingly outsourced to external foundries to reduce manufacturing costs, there has also been a much larger question of trust between design companies and the foundries, as there is the potential for introducing hardware Trojans during this process \cite{vashistha2018, varshney2020}. These Trojans consist of malicious changes performed on an IC's design and are inserted during manufacturing in order to implement a variety of attacks. Such attacks include sending information to outside sources, allowing an outside source to take control, or even disabling the functionality of a device using the infected IC. Obviously, hardware Trojans pose a potential security threat to their users, which can range from civilian to military applications, where security is absolutely essential for proper functionality. This potential risk has led to an interest in a rapid and accurate hardware Trojan detection system, which ideally would be able to identify the presence of a Trojan before an IC is put into use and can pose a greater risk.

\subsection{Hardware Security - Defenses: Traditional Methods}
%Destructive Methods
%In the past, destructive methods have generally been the most effective manner of finding hardware trojans.
Destructive methods have been used to effectively detect hardware Trojans traditionally. Usually, they require a complete reverse engineering of an IC, for which a few different processes have been developed, including a method proposed by Bao et. al. \cite{bao2015}. Through this method, an IC is completely decapsulated, polished, and imaged layer-by-layer to be compared to a Trojan-free golden layout of the same design. While generally producing very accurate results, this process also requires a large amount of time and resources, which often makes it ineffective for a rapid verification of ICs, especially when performed on a large scale.

Other destructive methods can include the use of a Focused Ion Beam (FIB). FIBs allow for the modification of a specimen with nanometer precision. Varshney et. al. \cite{varshney2020} introduced a Helium-ion FIB imaging method to accurately detect hardware Trojans found in ICs. This proposed method involves the etching, polishing, and ion milling of a 28-nm Xilinx Field-Programmable Gate Array (FPGA) until the p+ and n+ heavily doped silicon layer are exposed. By targeting the He-ion beam to certain regions of interest, filler cells can be detected. These filler cells are where adversaries can plant malicious insertions or delete the highly doped surrounding silicon with more filler cells, therefore essentially deactivating that part of the IC. Varshney et. al. proved how a He-ion FIB can be more useful than the SEM imaging processes. However, as in many of prior methods, the golden layouts of ICs should be available for this method.

%Non destructive methods
Other methods of Trojan detection have also included non-destructive procedures, which allow for Trojans to be found while keeping an IC intact. Side-channel analysis attempts to detect the presence of a Trojan by analysing the various physical characteristics of an IC, such as an effect on power usage, electromagnetic fields, and propagation delays \cite{hely2013}. While simpler to perform compared to the other methods, these methods are not always reliable due to the presence of noise and can even be prevented by the Trojan designer if designed in a certain fashion \cite{chakraborty2009}. Logic testing involves the creation of test patterns, designed to attempt in triggering a Trojan, which may be used in conjunction with side-channel analysis in certain conditions \cite{flottes2015}. The downside of this form of testing is that it is only able to identify Trojans that are designed to be triggered, and cannot identify those that run passively within an IC.

%Limitations
Despite the promise shown in each of these models, they all currently suffer from various limitations that make them less than ideal for a rapid and consistent Trojan detection framework. Reverse engineering is generally the most robust method, but it comes at a high cost due to the amount of time needed to image and analyze the layout of an IC, as well as to the associated cost of equipment and resources required to complete an entire analysis. Non-destructive methods by their nature avoid these problems and are generally less costly and labor intensive, but they are also not nearly as reliable. For instance, side-channel analysis can be susceptible to noise masking the presence of a Trojan \cite{chakraborty2009}, and logic testing can only be effective for a Trojan that is designed with a trigger, as opposed to one that is always running \cite{flottes2015}.

\subsection{Hardware Security - Defenses: Image Analysis-Based Methods}
The trade-off in cost and time versus accuracy between the destructive and non-destructive methods has previously been a problem for developing a reliable and cost-effective method of Trojan detection. However, with the increase in availability of electron microscope imaging as well as advances in the area of computer vision, there has been a growing shift towards using automated image analysis-based methods for this task as an alternative to the traditional methods. Generally, these methods attempt to automate the imaging and analysis process of reverse engineering, reducing the amount of time needed, and also maintaining most of the accuracy of a complete reverse engineering computation. Accordingly, many strides have been made towards creating a reliable system using image analysis.

%image matching
Continuing development in the field of computer vision has opened up many different ways of performing this image analysis. One way proposed by Courbon, et. al. \cite{courbon2015} made use of electron microscope images, and utilized simple image transform methods to straighten and match the dimensions of a control "golden" layout. The two images were then overlaid, which highlighted areas that differed between the two, especially those areas which were modified in order for a hardware Trojan to be inserted. Vashistha et. al. \cite{vashistha2018} also proposed a similar, but more advanced method of Trojan detection by obtaining high-quality golden layout images and using computer vision techniques for comparing the data to low-quality SEM images of an IC under authentication. For this method, image enhancement was performed on the SEM images and a structural similarity index was calculated on each pixel to highlight potentially modified areas.

%SVM, classical ML, K-means
An alternative method of image matching is the application of machine learning, a field which has gained much attention in recent years and has become mature enough to make significant improvements. In applying its techniques towards hardware security, specifically for the task of Trojan detection, Bao et. al. \cite{bao2014, bao2015} proposed leveraging Support Vector Machine (SVM) and K-means clustering. Both techniques used metal-layer SEM images as those taken in the reverse engineering process. Although both methods provided fairly accurate results, K-means clustering was found to have the benefits of reduced data over-fitting and more detailed classification about the type of modifications. On the other side, the SVM output showed simply whether a grid cell is infected or not. However, in a direct comparison K-means clustering was found to be slightly less accurate than the SVM approach, so there are certain trade-offs in their benefits.

%DL - segmentation, anomaly detection
Massive leaps in technology have also allowed for superior data acquisition in higher quality and quantities, while traditional machine learning algorithms are not suitable for large amounts of data \cite{wang2020}. However, deep learning has made large strides to be able to administer such data, and its techniques have been used to improve upon the prior image-matching methods through automatic analysis of larger amount of IC images, leading to getting higher accuracy. Hong et. al. \cite{hong2018} proposed a systematic training and validation approach using deep learning for IC image semantic segmentation. The proposed approach separated different IC image features into distinct regions of interest while providing noise cancellation on both the systematic and the irregular levels. This method resulted in obtaining low circuit annotation errors and high segmentation pixel accuracy. Cheng et. al. \cite{cheng2019} introduced a process of dividing an IC image based on its different geometries and using a hierarchical multi-classifier system trained on these shapes to identify the shapes within a given image, which were then merged to create complete IC segmentation. This approach was found to provide higher accuracy compared with the previous computer vision techniques and provided certain evidences for the usefulness for machine learning within IC analysis.

%DL - HT focus (i.e. Lin e.a.)

The emerging methods in Trojan detection have taken advantage of the novel deep learning concepts and ideas to develop remarkably rapid and accurate frameworks. In a related technique, Lin et. al. \cite{lin2020} proposed a deep learning image analysis framework for hardware assurance of digital ICs. The framework's objective was to inspect and authenticate various hardware information from extracted the SEM images. By utilizing a heavy use of deep learning-based methods, this framework aimed to reduce the time and efforts required in model re-training though employing diverse and automated (or semi-automated) data preparation methods. The proposed method by Lin et. al. was demonstrated to be fast, noise resistant, accurate, and capable of automating manual tasks. It was tested only on one set of images, therefore, parameters must be changed in order to accommodate for new sets of images.

%Image-based limitations?
One of the major issues of many of these image-based methods is that they rely on high-quality SEM images, in which the amounts of noise are limited, which increases the time needed for the SEM imaging process. Another issue is that a number of methods rely on having access to the golden layout of an IC as a control reference, which is often not available. However, there are certain methods that are able to slightly overcome this problem and perform Trojan detection without a golden layout. Additionally, for machine/deep learning-based methods, a large amount of training data is required to be acquired in order to fully train a model. The process of creating a data set with such a scale obviously enhances the needed time and labor immensely and is a major challenge for creating a rapid system.

%Conclusion - introduce our task
As a conclusive statement, large amounts of data should be available typically in order to effectively utilize deep learning concepts and techniques. For tackling this problem, we proposed leveraging a form of Generative Adversarial Network (GAN) to create synthetic cell/gate SEM images from real IC SEM images \cite{synthetic-sem-image}. Using the synthetic images, a defense system can be well strengthened in recognition of unique region-of-interests as well as the cells/gates of an IC. So, the system performance is improved in determination of whether the IC under test and authentication is trusted or not. Our proposed method and its experimental results are discussed in the following.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> random.tex <==
The block recognition unit works as a filter on what to pass to the rest of the process. The unit receives cells extracted from the SEM image the reference and the test cell SEM images for training and testing computations. The unit classifier outputs a probability distribution corresponding to the number of types/classes of IC cells and uses it to determine the appropriate class for a cell (which is specified based on the highest probability in the class vector). The registration of the reference cells is done during the training process using the image format of DEF layout file. The classifier output determines the validity of a cell in terms of the presence of its type in the original design. If a cell type was not present during the registration process or the image of a registered cell is changed sufficiently, then the classifier determines its status as "unknown" that means presence of an abnormal entity (malicious or non-malicious) in the design. The overall computational flow of block recognition unit is depicted in Figure \ref{fig:blk_det_recog}. A report containing the probabilities is generated from the recognition unit and is delivered to the decision-making unit.
